Computing obstructions for existence of connections on modules

We consider the notion of a connection on a module over a commutative ring, and recall the obstruction calculus for such connections. The obstruction calculus is defined using Hochschild cohomology. However, in order to compute with Grobner bases, we need the conversion to a description using free resolutions. We describe our implementation in Singular 3.0, available as the library conn.lib. Finally, we use the library to verify some known results and to obtain a new theorem for maximal Cohen-Macaulay (MCM) modules on isolated singularities. For a simple hypersurface singularity of dimension one or two, it is known that all MCM modules admit connections. We prove that for a simple threefold hypersurface singularity of type A_n, D_n or E_n, only the free MCM modules admit connections if n is at most 50.

==> obstr.tex <==

\section{Obstruction theory}
\label{s:obstr}

Let $k$ be an algebraically closed field of characteristic $0$, and
let $A$ be any commutative $k$-algebra. For any $A$-modules $M,M'$,
we refer to \citet{wei94} for the definition of the \emph{Hochschild
cohomology groups} $\hh^n(A, \hmm_k(M,M'))$ of $A$ with values in
the bimodule $\hmm_k(M,M')$. We recall that there is a natural
isomorphism of $k$-linear vector spaces $\ext^n_A(M,M') \to
\hh^n(A,\hmm_k(M,M'))$ for any $n \ge 0$. Furthermore, we shall
often use that there is an exact sequence of $k$-linear vector
spaces
\begin{multline} \label{s:hh}
0 \to \hh^0(A, \hmm_k(M,M')) = \hmm_A(M,M') \to \hmm_k(M,M') \\
\xrightarrow{\mu} \der_k(A, \hmm_k(M,M')) \to \hh^1(A, \hmm_k(M,M'))
\to 0,
\end{multline}
where $\mu$ is the assignment which maps $\phi \in \hmm_k(M,M')$ to
the trivial derivation given by $(a,m) \mapsto a \phi(m) - \phi(am)$
for all $a \in A, \; m \in M$.

Let $M$ be any $A$-module. We define a \emph{connection} on $M$ to
be a $k$-linear map $\nabla: M \to M \otimes_A \kdf A$ such that
$\nabla(am) = a\nabla(m) + m \otimes d(a)$ for all $a \in A$, $m \in
M$.

Let $\nabla$ be a connection on $M$. For any $D \in \der_k(A)$,
there is an induced $A$-linear map $\kdf A \to A$. It follows that
$\nabla$ induces a $k$-linear map $\nabla_D: M \to M$ with
derivation property with respect to $D$, i.e. $\nabla_D(am) = a
\nabla_D(m) + D(a) \, m$ for all $a \in A, \; m \in M$. We obtain an
$A$-linear map $\nabla: \der_k(A) \to \enm_k(M)$, which is called
the covariant derivation associated with the connection $\nabla$.
This construction motivates the following definitions:

A subset $\g \subseteq \der_k(A)$ is a \emph{Lie-Rinehart algebra} if
it is closed under the $A$-module and $k$-Lie algebra structures on
$\der_k(A)$, see \citet {ri63}. In this case, we define a
\emph{$\g$-connection} on $M$ to be an $A$-linear map $\nabla: \g \to
\enm_k(M)$ such that
    \[ \nabla_D(am) = a \nabla_D(m) + D(a) \, m \text{ for all } D
    \in \g, \; a \in A, \; m \in M. \]
If $\nabla: \g \to \enm_k(M)$ is only $k$-linear, then we shall call
$\nabla$ a $k$-linear $\g$-connection on $M$. When $\g = \der_k(A)$,
we shall refer to a $\g$-connection (or covariant derivation) simply
as a connection.

\begin{prop} \label{p:ksker}
There is a canonical map $g: \der_k(A) \to \ext^1_A(M,M)$, called
the Kodaira-Spencer map of $M$, with the following properties:
\begin{enumerate}
\item The Kodaira-Spencer kernel $\ksker(M) = \ker(g)$ is
a Lie algebroid of $A/k$,
\item For any $D \in \der_k(A)$, there exists an operator $\nabla_D
\in \enm_k(M)$ with derivation property with respect to $D$ if and only
if $D \in \ksker(M)$.
\end{enumerate}
In particular, $\ksker(M)$ is maximal among the subsets $\g
\subseteq \der_k(A)$ such that there exists a $k$-linear
$\g$-connection on $M$.
\end{prop}
\begin{pf}
Let $\psi_D \in \der_k(A, \enm_k(M))$ be given by $\psi_D(a)(m) =
D(a) \, m$ for any $D \in \der_k(A)$, and denote by $g(D)$ the class
in $\ext^1_A(M,M)$ corresponding to the class of $\psi_D$ in
$\hh^1(A, \enm_k(M))$. This defines the Kodaira-Spencer map $g$ of
$M$, which is $A$-linear by definition. Clearly, its kernel
$\ksker(M)$ is closed under the Lie product. Using the exact
sequence (\ref{s:hh}), it easily follows that there exists an
operator $\nabla_D$ with derivation property with respect to $D$ if
and only if $D \in \ksker(M)$.
\end{pf}

We remark that the map $g$ in the proof of proposition \ref{p:ksker} is
the contraction against the first Atiyah class of the $A$-module $M$.
It is therefore well-known that $g$ is the Kodaira-Spencer map of $M$,
see \citet{ill71, ill72}. See also \citet{kal05}, section 2.2 for
another proof of proposition \ref{p:ksker}.

\begin{prop} \label{p:lc}
There is a canonical class $\lc(M) \in \ext^1_A(\ksker(M), \enm_A(M))$
such that $\lc(M) = 0$ if and only if there exists a
$\ksker(M)$-connection on $M$. Moreover, if $\lc(M) = 0$, then there is
a transitive and effective action of $\hmm_A(\ksker(M), \enm_A(M))$ on
the set of $\ksker(M)$-connections on $M$.
\end{prop}
\begin{pf}
Let $\ksker = \ksker(M)$, choose a $k$-linear $\ksker$-connection
$\nabla: \ksker \to \enm_k(M)$ on $M$, and let $\phi \in \der_k(A,
\hmm_k(\ksker, \enm_A(M)))$ be the derivation given by $\phi(a)(D) =
a \nabla_{D} - \nabla_{aD}$. We denote by $\lc(M)$ the class in
$\ext^1_A(\ksker, \enm_A(M))$ corresponding to the class of $\phi$
in $\hh^1(A, \hmm_k(\ksker, \enm_A(M)))$, and it is easy to check
that this class is independent of $\nabla$. Using the exact sequence
(\ref{s:hh}), the proposition follows easily.
\end{pf}

There is a natural short exact sequence $0 \to \enm_A(M) \to c(M) \to
\ksker(M) \to 0$ of left $A$-modules, where $c(M) = \{ \phi \in
\enm_k(M): [\phi,a] \in A \text{ for all } a \in A \}$ is the module of
first order differential operators on $M$ with scalar symbol. We remark
that $c(M)$ represents $\lc(M)$ as an extension of $A$-modules, see
also \citet{kal05}, proposition 2.2.10.

\begin{lem} \label{l:dirsum}
For any $A$-modules $M,M'$, we have $\ksker(M \oplus M') = \ksker(M)
\cap \ksker(M')$, and $\lc(M \oplus M') = 0$ if and only if $\lc(M)
= \lc(M') = 0$.
\end{lem}

Lemma \ref{l:dirsum} is a direct consequence of proposition
\ref{p:ksker} and \ref{p:lc}. We remark that the first part also
follows from \citet{bu-li04}, lemma 3.4.



\section{Computing with free resolutions}
\label{s:freeres}

It is convenient to use Hochschild cohomology to define the
obstruction theory and deduce its basic properties, as we have done
in section \ref{s:obstr}. However, in order to compute the
obstructions effectively using Gr\"obner bases in {\sc Singular}, we
shall use free resolutions. We have already seen that there are
isomorphisms of $k$-linear vector spaces
    \[ \ext^n_A(M,M') \to \hh^n(A,\hmm_k(M,M')) \]
for all $n \ge 0$. For our purposes, it is crucial to find a more
explicit version of this identification in the case $n = 1$.

Let $(L_{\cpd}, d_{\cpd})$ be a free resolution of $M$, and let
$\tau: M \to L_0$ be a $k$-linear section of the augmentation
morphism $\rho: L_0 \to M$. Let moreover $\phi: L_1 \to M'$ be a
$1$-cocyle in $\hmm_A(L_{\cpd}, M')$. For any $a \in A, \; m \in M$,
we can find an element $x = x(a,m) \in L_1$ such that $d_0(x) = a
\tau(m) - \tau(am)$. It is easy to check that $\psi(a)(m) = \phi(x)$
defines a derivation $\psi \in \der_k(A, \hmm_k(M,M'))$ which is
independent of the choice of $x$.

\begin{lem} \label{l:id}
The assignment $\phi \mapsto \psi$ defined above induces a natural
injective map $\sigma: \ext^1_A(M,M') \to \hh^1(A, \hmm_k(M,M'))$ of
$k$-linear vector spaces.
\end{lem}
\begin{pf}
If $\phi = \phi' d_0$ is a coboundary in $\hmm_A(L_{\cpd},M')$, then
$\psi$ is a trivial derivation, given by $\psi(a)(m) = a \psi'(m) -
\psi'(am)$ with $\psi' = \phi' \tau$. Hence the assignment induces a
well-defined map $\sigma$ of $k$-linear vector spaces. To see that
it is injective, assume that $\phi$ is a $1$-cocyle in
$\hmm_A(L_{\cpd}, M')$ which maps to a trivial derivation $\psi$,
given by $\psi(a)(m) = a \psi'(m) - \psi'(am)$ for some $\psi' \in
\hmm_k(M,M')$. For any $x \in L_0$, there exists an element $x' \in
L_1$ such that $d_0(x') = x - \tau \rho(x)$, and $x'$ is unique
modulo $\im(d_1)$. Let us define $\phi': L_0 \to M'$ to be the map
given by $\phi'(x) = \psi' \rho(x) + \phi(x')$, this is clearly a
well-defined map since $\phi \, d_1 = 0$. One may show that $\phi'$
is $A$-linear, and it satisfies $\phi' d_0 = \phi$ by construction.
Hence $\phi$ is a coboundary.
\end{pf}

Let $k$ be an algebraically closed field of characteristic $0$, let
$A$ be a commutative $k$-algebra essentially of finite type, and let
$M$ be a finitely generated $A$-module. Then we can find a free
resolution
    \[ 0 \gets M \xleftarrow{\rho} L_0 \xleftarrow{d_0} L_1
    \gets \dots \]
of $M$ such that $L_i$ has finite rank for all $i \ge 0$. Let us choose
isomorphisms $L_0 \cong A^m$ and $L_1 \cong A^n$, and write $( a_{ij}
)$ for the matrix of $d_0: L_1 \to L_0$ with respect to the chosen
bases. One may show that for any $D \in \der_k(A)$, the matrix $(
D(a_{ij}) )$, considered as an $A$-linear map $L_1 \to L_0$, defines a
$1$-cocycle in $\hmm_A(L_{\cpd},M)$ and therefore a cohomology class
$g(D)'$ in $\ext^1_A(M,M)$. From the explicit form of the first Atiyah
class given in \citet{an-lj89}, we see that the map $D \mapsto g(D)'$
is the contraction against this class.

Since $A$ is essentially of finite type over $k$, it follows that
$\ksker(M)$ is a left $A$-module of finite type. Then we can find a
free resolution of $\ksker(M)$ as a left $A$-module
    \[ 0 \gets \ksker(M) \xleftarrow{\rho'} L'_0 \xleftarrow{d'_0}
    L'_1 \gets \dots \]
such that $L'_i$ has finite rank for all $i \ge 0$. Let us choose
isomorphisms $L'_0 \cong A^p$ and $L'_1 \cong A^q$, and write $( c_{ij}
)$ for the matrix of $d'_0: L'_1 \to L'_0$ with respect to the chosen
bases. For $1 \le i \le p$, let us write $D_i = \rho'(e_i)$. Since $D_i
\in \ksker(M)$, we can find a $k$-linear operator $\nabla_i$ on $M$
which has the derivation property with respect to $D_i$ by proposition
\ref{p:ksker}. One may show that $\nabla_i$ can be lifted to an
operator on $L_0 \cong A^m$ of the form $D_i^m + P_i$, where $D_i^m:
A^m \to A^m$ operates component by component, and $P_i: A^m \to A^m$ is
an $A$-linear operator. This means that $R_j = \sum c_{ij} P_i$ induces
an $A$-linear operator on $M$ for $1 \le j \le q$. One may show that
the $A$-linear map $L'_1 \to \enm_A(M)$ given by $e_j \mapsto R_j$ is a
$1$-cocycle in $\hmm_A(L'_{\cpd}, \enm_A(M))$, and therefore defines a
cohomology class $\lc(M)'$ in $\ext^1_A(\ksker(M), \enm_A(M))$.

The following lemma follows from more general results, see for instance
\citet{bu-fl03}. For completeness, we include an elementary proof:

\begin{lem} \label{l:idobstr}
We have that
\begin{enumerate}
\item $g(D) = 0$ if and only if $g(D)' = 0$,
\item $\lc(M) = 0$ if and only if $\lc(M)' = 0$.
\end{enumerate}
\end{lem}
\begin{pf}
Since $\sigma$ is injective, it is enough to show that $\sigma$ maps
$g(D)'$ to $g(D)$ and $\lc(M)'$ to $\lc(M)$. To show that $g(D)'
\mapsto g(D)$, it is enough to notice that $( D(a_{ij}) ) = D^m d_0
- d_0 D^n$, where $D^m$ and $D^n$ operates component by component on
$A^m$ and $A^n$. To show that $\lc(M)' \mapsto \lc(M)$, consider the
$A$-linear map $\nabla: A^p \to \enm_k(M)$ given by $e_i \mapsto
\nabla_i$ for $1 \le i \le p$, and notice that $\nabla d'_0(e_j) =
R_j$ for $1 \le j \le q$ and that $\nabla \tau'$ is a $k$-linear
$\ksker(M)$-connection on $M$ for any $k$-linear section $\tau'$ of
$\rho'$. For any $a \in A, \; D \in \ksker(M)$, choose $x \in L'_1$
such that $d'_0(x) = a \tau'(D) - \tau'(aD)$. Then the cocycle $e_j
\mapsto R_j$ maps $x$ to $\nabla(a \tau'(D) - \tau'(aD)) = a \nabla
\tau'(D) - \nabla \tau'(aD)$. By definition of $\sigma$, it follows
that $\lc(M)' \mapsto \lc(M)$.
\end{pf}

